A Faster Algorithm for Finding Closest Pairs in Hamming Metric

We study the Closest Pair Problem in Hamming metric, which asks to find the pair with the smallest Hamming distance in a collection of binary vectors. We give a new randomized algorithm for the problem on uniformly random input outperforming previous approaches whenever the dimension of input points is small compared to the dataset size. For moderate to large dimensions, our algorithm matches the time complexity of the previously best-known locality sensitive hashing based algorithms. Technically our algorithm follows similar design principles as Dubiner (IEEE Trans. Inf. Theory 2010) and May-Ozerov (Eurocrypt 2015). Besides improving the time complexity in the aforementioned areas, we significantly simplify the analysis of these previous works. We give a modular analysis, which allows us to investigate the performance of the algorithm also on non-uniform input distributions. Furthermore, we give a proof of concept implementation of our algorithm which performs well in comparison to a quadratic search baseline. This is the first step towards answering an open question raised by May and Ozerov regarding the practicability of algorithms following these design principles.

==> imgs/algorithm_fill.tex <==
\usetikzlibrary{patterns,decorations.pathreplacing}

\begin{tikzpicture}

% List 1
\draw [draw] (0,0) -- (-1.5,0) -- (-1.5,7.5) -- (0,7.5) -- (0,0);
\node at (-0.8,7.7) {$L_1$};
\pattern[pattern=north east lines] (-1.5,5.5) -- (0,5.5) -- (0,1.5) -- (-1.5,1.5) --cycle;
\draw  (-1.5,5.5) edge (0,5.5);
\draw  (-1.5,1.5) edge (0,1.5);
\node at (-0.7,5.7) {$\mathrm{wt} = \delta n$};

%brace links
\draw [decorate,decoration={brace,amplitude=3pt},xshift=0pt,yshift=0pt]
(-1.6,0) -- (-1.6,7.5) node [black,midway,xshift=-0.6cm] 
{\footnotesize $2^{\lambda n}$};
%brace unten
\draw [decorate,decoration={brace,amplitude=3pt},xshift=0pt,yshift=0pt]
(0,-0.1) -- (-1.5,-0.1) node [black,midway,yshift=-0.3cm] 
{\footnotesize $n$};

% arrows for r = 0 -> 1
\draw [->] (0,3.5) -- (1.5,6);
\draw [->] (0,3.5) -- (1.5,1.5);
\node at (1,6) {$1$};
\node at (1,1) {$N$};
\path (1,5) -- node[auto=false]{\vdots} (1,2.2);
\path (1.5,3.5) -- node[auto=false]{\dots} (3,4);

% list r = 1 N = 1
\draw [draw](0,0) (1.5,8) -- (3,8) -- (3,4) -- (1.5,4) -- (1.5,8);
% uncomment this line to fill the whole square with a dashed area
%\pattern[pattern=north east lines] (1.5,8.5) --(3,8.5) --(3,4.5) --(1.5,4.5)--cycle;
\pattern[pattern=north west lines, dotted] (1.5,7) --(3,7) -- (3,5) -- (1.5,5) --cycle;
\draw [draw] (1.5,7) -- (3,7);
\draw (1.5,5) -- (3,5);

% arrows for N = 1, r = 1 -> 2
\draw [->] (3,6) -- (4,7);
\draw [->] (3,6) -- (4,5);
\node at (3.5,7) {$1$};
\node at (3.5,5) {$N$};
\path (4,5) -- node[auto=false]{\vdots} (4,7);


% list r = 1 N = N
\draw [draw](0,0) (1.5,-0.5) -- (3,-0.5) -- (3,3.5) -- (1.5,3.5) -- (1.5,-0.5);
% uncomment this line to fill the whole square with a dashed area
%\pattern[pattern=north east lines] (1.5,8.5) --(3,8.5) --(3,4.5) --(1.5,4.5)--cycle;
\pattern[pattern=north west lines, dotted] (1.5,0.5) -- (3,0.5) -- (3,2.5) -- (1.5,2.5) --cycle;
\draw [draw] (1.5,0.5) -- (3,0.5);
\draw (1.5,2.5) -- (3,2.5);

% arrows for N = N, r = 1 -> 2
\draw [->] (3,1.5) -- (4,0.5);
\draw [->] (3,1.5) -- (4,2.5);
\node at (3.5,2.5) {$1$};
\node at (3.5,0.5) {$N$};
\path (4,2.5) -- node[auto=false]{\vdots} (4,0.5);

% dots between layer 2 and r
\path (4,7) -- node[auto=false]{\dots} (5,7);
\path (4,3.7) -- node[auto=false]{\dots} (5,3.7);
\path (4,0.5) -- node[auto=false]{\dots} (5,0.5);


% Final Tabel
%\pattern[pattern=north west lines, dotted] (7,3.5) node (v12) {}  --(5.5,3.5) --(5.5,5.5) node (v10) {}  --(7,5.5) node (v11) {} --cycle;
\draw (7,5.5) -- (8.5,5.5) -- (8.5,3.5) -- (7,3.5) -- (7,5.5);
\draw [->] (6,4) -- (7,4.5);
\draw [line width=2pt](7,5) -- (8.5,5);
\node at (7.7,5.2) {$\mathbf x$};

% Final buttom line of r 
\node at (-2,-1.5) {$r:$};
\node at (-1,-1.5) {$0$};
\node at (2.3,-1.5) {$1$};
\node at (7.5,-1.5) {$r$};

\end{tikzpicture}

==> imgs/algorithm_windowed.tex <==
\usetikzlibrary{patterns,decorations.pathreplacing}

\begin{tikzpicture}

% List 1
\draw [draw](1.5,0) node (v1) {} -- (-1.5,0) -- (-1.5,7.5) -- (1.5,7.5) -- (v1);
\node at (0,9) {$L_1$};
\pattern[pattern=north east lines] (-1.5,5.5) node (v2) {}--(1.5,5.5) node (v3) {}--(1.5,1.5) node (v5) {}--(-1.5,1.5) node (v4) {}--cycle;
\pattern[pattern=north west lines] (-1.5,0) node (v2) {}--(-0.5,0) node (v3) {}--(-0.5,7.5) node (v5) {}--(-1.5,7.5) node (v4) {}--cycle;

\draw  (v2) edge (v3);
\draw  (v4) edge (v5);
\draw (v5) edge (v3);

%brace ganz oben
\draw [decorate,decoration={brace,amplitude=3pt},xshift=0pt,yshift=0pt]
(-1,8.2) -- (1.5,8.2) node [black,midway,yshift=+0.3cm] 
{\footnotesize $r$};

%brace oben
\draw [decorate,decoration={brace,amplitude=3pt},xshift=0pt,yshift=0pt]
(-1.5,7.6) -- (-0.5,7.6) node [black,midway,yshift=+0.3cm] 
{\footnotesize $k = \frac{n}{r}$};

%brace links
\draw [decorate,decoration={brace,amplitude=3pt},xshift=0pt,yshift=0pt]
(-1.6,0) -- (-1.6,7.5) node [black,midway,xshift=-0.6cm] 
{\footnotesize $2^{\lambda n}$};

%brace unten
\draw [decorate,decoration={brace,amplitude=3pt},xshift=0pt,yshift=0pt]
(1.5,-0.1) -- (-1.5,-0.1) node [black,midway,yshift=-0.3cm] 
{\footnotesize $n$};

\draw (-1.5,5.5) -- (1.5,5.5);
\draw (-1.5,1.5) -- (1.5,1.5);

% Text und gewicht
\node at (0.5,6.6) {$\mathrm{wt} = \delta k$};
\draw (-1.5,1.5) -- (1.5,1.5);




% List 2
\draw [draw](16,0) node (v1) {} -- (13,0) -- (13,7.5) -- (16,7.5) -- (v1);
\node at (14,9) {$L_2$};
\pattern[pattern=north east lines] (16,5) node (v2) {}--(13,5) node (v3) {}--(13,2.5) node (v5) {}--(16,2.5) node (v4) {}--cycle;
\pattern[pattern=north west lines] (13,0) node (v2) {}--(14,0) node (v3) {}--(14,7.5) node (v5) {}--(13,7.5) node (v4) {}--cycle;

\draw  (13,5) edge (16,5);
\draw  (13,2.5) edge (16,2.5);
\draw  (14,0) edge (14,7.5);

%brace rechts
\draw [decorate,decoration={brace,amplitude=3pt},xshift=0pt,yshift=0pt]
(16.1,7.5) -- (16.1,0) node [black,midway,xshift=+0.6cm] 
{\footnotesize $2^{\lambda n}$};


% liste oben.
\draw (3,9) node (v6) {} -- (6,9) -- (6,4.5) -- (3,4.5) -- (v6);
\draw [->](1.5,4.5) -- (3,7);
\draw [->](1.5,4.5) -- (3,2.5);
\node at (2.5,6.5) {$1$};
\node at (2.5,3) {$N$};

\pattern[pattern=north east lines] (6,8) node (v10) {} --(3,8) node (v9) {} --(3,6) node (v11) {} --(6,6) --cycle;
\pattern[pattern=north west lines] (5,4.5) node (vbla8) {}--(4,4.5) --(4,9) node (v8) {} --(5,9) node (v7) {} --cycle;

\draw (v7) -- (vbla8.mid);
\draw (v9) -- (v10);
\draw (v11) -- (6,6);
\draw (v8) -- (4,4.5);

% Listen unten.
\draw (8.5,4) -- (11.5,4) -- (11.5,-0.5) -- (8.5,-0.5) -- (8.5,4);
\draw [->](13,3.5) -- (11.5,2);
\draw [->](13,3.5) -- (11.5,5.5);
\node at (12,5) {$1$};
\node at (12,2) {$N$};
\pattern[pattern=north east lines] (8.5,1.5) node (v2) {}--(11.5,1.5) node (v3) {}--(11.5,0) node (v5) {}--(8.5,0) node (v4) {}--cycle;
\draw (v2) -- (v3);
\draw (v4) -- (v5);
\pattern[pattern=north west lines] (10.5,-0.5) node (v2) {}--(9.5,-0.5) node (v3) {}--(9.5,4) node (v5) {}--(10.5,4) node (v4) {}--cycle;
\draw (v4) -- (v2);
\draw (v5) -- (v3);




\end{tikzpicture}

==> imgs/algorithm_windowed_singlelist.tex <==
\usetikzlibrary{patterns,decorations.pathreplacing}

\begin{tikzpicture}

% List 1
\draw [draw](1.5,0.5) -- (-1.5,0.5) -- (-1.5,7.5) -- (1.5,7.5) -- (1.5,0.5);
\node at (0,9) {$L_1$};
\pattern[pattern=north east lines] (-1.5,5.5) -- (1.5,5.5) -- (1.5,1.5) -- (-1.5,1.5) -- cycle;
\pattern[pattern=north west lines] (-1.5,0.5) -- (-0.8,0.5) -- (-0.8,7.5) -- (-1.5,7.5) -- cycle;

\draw  (-1.5,5.5) edge (1.5,5.5);
\draw  (-1.5,7.5) edge (-0.8,7.5);
\draw (-0.8,7.5) edge  (-0.8,0.5);

%brace ganz oben
\draw [decorate,decoration={brace,amplitude=3pt},xshift=0pt,yshift=0pt]
(-1,8.2) -- (1,8.2) node [black,midway,yshift=+0.3cm] 
{\footnotesize $r$};

%brace oben
\draw [decorate,decoration={brace,amplitude=3pt},xshift=0pt,yshift=0pt]
(-1.5,7.6) -- (-0.8,7.6) node [black,midway,yshift=+0.3cm] 
{\footnotesize $k = \frac{n}{r}$};

%brace links
\draw [decorate,decoration={brace,amplitude=3pt},xshift=0pt,yshift=0pt]
(-1.6,0.5) -- (-1.6,7.5) node [black,midway,xshift=-0.4cm] 
{\footnotesize $2^{\lambda n}$};

%brace unten
\draw [decorate,decoration={brace,amplitude=3pt},xshift=0pt,yshift=0pt]
(1.5,0.4) -- (-1.5,0.4) node [black,midway,yshift=-0.3cm] 
{\footnotesize $n$};

\draw (-1.5,5.5) -- (1.5,5.5);
\draw (-1.5,1.5) -- (1.5,1.5);

% Text und gewicht
\node at (0.5,6.6) {$\mathrm{wt} = \delta k$};
\draw [->](-0.1,6.4) -- (-0.9,5.3);
\draw (-1.5,1.5) -- (1.5,1.5);


% Layer2
% Pfeile
\draw [->](1.5,4) -- (3,6);
\draw [->](1.5,4) -- (3,2);
\node at (2.5,6) {$1$};
\node at (2.5,2) {$N$};
\path (2.5,5.5) -- node[auto=false]{\vdots} (2.5,2.5);

%dots zwischen liste 1 .2
\path (4.5,4.5) -- node[auto=false]{\vdots} (4.5,3.5);

% liste oben.
\draw (3,8.5) -- (6,8.5) -- (6,4.5) -- (3,4.5) -- (3,8.5);
\pattern[pattern=north east lines] (6,7.8) -- (3,7.8) -- (3,5.7) --(6,5.7) --cycle;
\pattern[pattern=north west lines] (4.4,4.5) --(3.7,4.5) -- (3.7,8.5) -- (4.4,8.5) --cycle;

\draw (4.4,8.5) -- (4.4,4.5);
\draw (3,7.8) -- (6,7.8);
\draw (3,5.7) -- (6,5.7);
\draw (3.7,8.5) -- (3.7,4.5);

% Liste Unten
\draw (3,-0.5) -- (6,-0.5) -- (6,3.5) -- (3,3.5) -- (3,-0.5);
\pattern[pattern=north east lines] (6,0) -- (3,0) -- (3,1.5) -- (6,1.5) --cycle;
\pattern[pattern=north west lines] (4.4,3.5) --(3.7,3.5) -- (3.7,-0.5) -- (4.5,-0.5) --cycle;

\draw (4.5,-0.5) -- (4.4,3.5);
\draw (3,0) -- (6,0);
\draw (3,1.5) -- (6,1.5);
\draw (3.7,-0.5) -- (3.7,3.5);

% Layer 3
%\path (7,5.5) -- node[auto=false]{\vdots} (7,2.5);

% Pfeile Oben
\draw [->](6,6.5) -- (7.5,7.5);
\draw [->](6,6.5) -- (7.5,5.5);
\path (7,7.5) -- node[auto=false]{\vdots} (7,5.5);
\path (8.5,7.5) -- node[auto=false]{\dots} (7.5,7.5);
\node at (7,7.5) {$1$};
\node at (7,5.5) {$N$};

% pfeile unten
\draw [->](6,1.5) -- (7.5,2.5);
\draw [->](6,1.5) -- (7.5,0.5);
\path (7,2.5) -- node[auto=false]{\vdots} (7,0.5);
\path (8.5,0.5) -- node[auto=false]{\dots} (7.5,0.5);
\node at (7,2.5) {$1$};
\node at (7,0.5) {$N$};

% Layer r
\draw [->](7.2,3.9) -- (8.7,4.6);

% Final List
\draw (11.7,3.9) -- (8.7,3.9) -- (8.7,5.4) -- (11.7,5.4) -- (11.7,3.9);
% auskommentiert da letzte liste
%\pattern[pattern=north east lines] (8.5,2.5) -- (11.5,2.5) -- (11.5,4) -- (8.5,4) --cycle;
\pattern[pattern=north west lines] (11,5.4) --(11.7,5.4) -- (11.7,3.9) -- (11,3.9) --cycle;

\draw (11.7,3.9) -- (11.7,5.4);
\draw (11,3.9) -- (11,5.4);
% auskommentiert da letzte liste.
%\draw (11.5,2.5) -- (8.5,2.5);
%\draw (11.5,4) -- (8.5,4);

% Final Solution
\draw [line width=2pt](8.7,4.9) -- (11.7,4.9);
\node at (10.2,5.1) {$\mathbf x$};

% Level bar
\node at (-2,-1) {Level:};
\node at (0,-1) {$1$};
\node at (4.5,-1) {$2$};
\node at (10,-1) {$r$};

\end{tikzpicture}
